"I'm Not Mad": Commonsense Implications of Negation and Contradiction

Natural language inference requires reasoning about contradictions, negations, and their commonsense implications. Given a simple premise (e.g., "I'm mad at you"), humans can reason about the varying shades of contradictory statements ranging from straightforward negations ("I'm not mad at you") to commonsense contradictions ("I'm happy"). Moreover, these negated or contradictory statements shift the commonsense implications of the original premise in nontrivial ways. For example, while "I'm mad" implies "I'm unhappy about something," negating the premise (i.e., "I'm not mad") does not necessarily negate the corresponding commonsense implications. In this paper, we present the first comprehensive study focusing on commonsense implications of negated statements and contradictions. We introduce ANION1, a new commonsense knowledge graph with 624K if-then rules focusing on negated and contradictory events. We then present joint generative and discriminative inference models for this new resource, providing novel empirical insights on how logical negations and commonsense contradictions reshape the commonsense implications of their original premises.

==> sections/7-related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Commonsense Knowledge Models}

% Specifically proposed a set of neural network models
% for scoring tuples in ConceptNet. Our work differs
% from this approach as their models evaluate full tuples
% rather than learning to generate the phrases to
% make new nodes in the knowledge graph.


Recent approaches have investigated how to distill commonsense knowledge from deep neural language models. 

% \citet{sap2019atomic} build LSTM encoder-decoder models to generate new commonsense knowledge tuples for the ATOMIC KB.

\citet{li-etal-2016-commonsense} assign quality scores to novel tuples in ConceptNet to distinguish true knowledge from false knowledge. However, they investigate how to use neural models to validate proposed knowledge rather than generating to expand the KB.
% develop neural network models to embed terms and provide scores to arbi-trary tuple, on-the-fly CKB completion model to improve the coverage of CKBs. defined the CKB completion task as a binary classification distinguishing true knowledge from false knowledge for arbitrary triples.

% One common way of improving the coverage of knowledge bases is through knowledge base com- pletion (KBC), which can be formalized as pre- dicting the existence of edges between (usually) pre-existing nodes in the graph. 

\citet{saito-etal-2018-commonsense} propose a joint learning method that incorporate generated knowledge tuples to augment their KB completion model, rather than to enrich the commonsense KB.

% builds upon this work by proposing a
% joint model for completion and generation of commonsense
% tuples. Their work, however, focuses on
% using tuple generation to augment their KB completion
% model, rather than to increase coverage in
% commonsense KB construction.


% we focus on problems of increas- ing the node size of CKBs and increasing the con- nectivity of CKBs. We introduce a new common- sense knowledge base generation (CKB genera- tion) task for generating new nodes. We also de- vise a model that jointly learns the completion and generation tasks.



\citet{jastrzebski-etal-2018-commonsense} extend these approaches to automatically mine commonsense knowledge from Wikipedia.
% improve the coverage of such resources

% More recent work mapped commonsense tuples to natural language
% with templates and used pretrained language models
% to validate them


% \citet{bosselut2019comet} use transformers and investigate the effect
% of using pretrained language representations to initialized commonsense knowledge representations. Concurrently, other research has explored using
% pretrained language models and adapting them as generative knowledge graph constructors


\citet{cui2020does} propose two attention-based methods to analyze commonsense knowledge inside BERT, and the contribution of such knowledge for the model prediction. We find that attention heads successfully capture the structured commonsense knowledge encoded in CONCEPTNET, which helps BERT solve commonsense tasks directly. Fine-tuning fur- ther makes BERT learn to use the common- sense knowledge on higher layers.


% \citet{bosselut2020dynamic} In contrast to these works that augment static
% knowledge graphs, our approach focuses on constructing
% knowledge graphs on demand to provide context-dependent
% commonsense for downstream inference.
% In this paper, we present initial studies toward zero-shot commonsense
% question answering by formulating the task as inference
% over dynamically generated commonsense knowledge
% graphs. In contrast to previous studies for knowledge integration
% that rely on retrieval of existing knowledge from static
% knowledge graphs, our study requires commonsense knowledge
% integration where contextually relevant knowledge is
% often not present in existing knowledge bases. Therefore, we
% present a novel approach that generates contextually-relevant
% symbolic knowledge structures on demand using generative
% neural commonsense knowledge models.


\citet{davison-etal-2019-commonsense} develop a method for generating commonsense knowledge using a large, pre-trained bidirectional language model. By transforming relational tuples into masked sentences, we can use this model to rank a tuple’s validity by the estimated pointwise mutual information between the two entities.
 Since we do not update the weights of the bidirectional model, our approach is not bi- ased by the coverage of any one common- sense knowledge base. Though this method performs worse on a test set than models ex- plicitly trained on a corresponding training set, it outperforms these methods when mining commonsense knowledge from new sources, suggesting that unsupervised techniques may generalize better than current supervised ap- proaches.


use a masked language model to estimate point-wise mutual information between entities in a possible relation,

\citet{klein-nabi-2020-contrastive} We propose a self-supervised method to
solve Pronoun Disambiguation and Winograd
Schema Challenge problems. Our approach
exploits the characteristic structure of training
corpora related to so-called “trigger” words,
which are responsible for flipping the answer
in pronoun disambiguation. We achieve such
commonsense reasoning by constructing pair-
wise contrastive auxiliary predictions. To this
end, we leverage a mutual exclusive loss regu-
larized by a contrastive margin. Our architec-
ture is based on the recently introduced trans-
former networks, BERT, that exhibits strong
performance on many NLP benchmarks. Em-
pirical results show that our method allevi-
ates the limitation of current supervised ap-
proaches for commonsense reasoning. 



% \cite{rajani2019explain} We collect human explanations for commonsense reason- ing in the form of natural language sequences and highlighted annotations in a new dataset called Common Sense Explanations (CoS-E). We use CoS-E to train language models to automatically generate explanations that can be used during training and inference in a novel Commonsense Auto-Generated Expla- nation (CAGE) framework. CAGE improves the state-of-the-art by 10\% on the challeng- ing CommonsenseQA task. We further study commonsense reasoning in DNNs using both human and auto-generated explanations in- cluding transfer to out-of-domain tasks. Em- pirical results indicate that we can effectively leverage language models for commonsense reasoning.




\paragraph{Natural Language Inference}

\citep{warstadt-etal-2019-investigating} 



% For NLI, talk about RTE task, SNLI, Multi-NLI, works by Ellie Pavlick, works by Sam Bowman, works by Tal Linzen, works by Benjamin Van Durme and Rachel Rudinger

% commonsense KB reasoning



==> sections/Z4-model.tex <==
\section{Commonsense Knowledge Model of Negated Events}
\label{sec:model}

In this section, we first introduce COMET \cite{bosselut2019comet}, the base commonsense knowledge generation model we focus on to study commonsense negation reasoning and a negation discriminator submodule used to identify logically plausible COMET generations.

\subsection{COMET}
\label{sec:model-comet}

\textbf{COM}mons\textbf{E}nse \textbf{T}ransformers (COMET) are generative commonsense knowledge models that learn to adapt a language model by training on a seed set of knowledge tuples.
Specifically, COMET consumes knowledge tuples in $\{h,r,t\}$ form during training, where $h$ is a head entity, $r$ is a relation type, and $t$ is a tail entity. In \atomic{}, head entities correspond to events, such as ``PersonX has a nightmare,'' and tail entities correspond to commonsense inferences about those events, such as ``As a result, PersonX wakes up.'' The relation types are various dimensions of commonsense inferences that can be made about the events. During the generation, COMET is given $h$ and $r$ to predict $t$.

%We adopt the same notation from \citet{bosselut2019comet}: $X^{h} = \{x_{0}^{h},...,x_{|h|}^{h}\}$ as tokens comprising the event, $X^{r} = \{x_{0}^{r},...,x_{|r|}^{r}\}$ as tokens comprising the relation, and $X^{t} = \{x_{0}^{t},...,x_{|t|}^{t}\}$ as tokens comprising the condition object. 

\paragraph{Input}

We use the same input token setup for training configurations as in \citet{bosselut2019comet}. A knowledge triple $\{h,r,t\}$ is represented as a concatenated sequence with tokens of each element in the tuple: $X = \{X^{h}, X^{r}, X^{y}\}$ where $X^{h} = \{x_{0}^{h},...,x_{|h|}^{h}\}$ are the tokens comprising the event, $X^{r} = \{x_{0}^{r},...,x_{|r|}^{r}\}$ as tokens comprising the relation, and $X^{t} = \{x_{0}^{t},...,x_{|t|}^{t}\}$ are the tokens comprising the commonsense inference. %During concatenation, we pad $X^{h}$ component to 21 tokens, which is the length of the longest events in the overall \atomic{} dataset, and pad $X^{t}$ to 44 tokens, the length of the longest condition object. 

\paragraph{Loss Function}

We train COMET to maximize the conditional loglikelihood of predicting the tokens of the commonsense inference, $X^{t}$:

\begin{equation}
\mathcal{L}_{C} = - \sum_{s=|h|+|r|}^{|h|+|r|+|t|} \log{P(x_{s}|x_{<s})}
\label{eq:comet-loss}
\end{equation}

\noindent where $|h|$, $|r|$, and $|t|$ are the length of the event, the relation type, and condition object, respectively.

\paragraph{Initialization}
Similar to \citet{bosselut2020dynamic}, we initialize the trained parameters of COMET to the 345M parameter GPT2 model (GPT2-M) from \citet{Radford2019LanguageMA}.%, with 24 layers and 1024-dimensional hidden states, resulting in 355M weights in total. 
Special tokens that represent relation types (e.g., ``xIntent'') are added to the vocabulary and initialized via sampling from the normal distribution.

\paragraph{Hyperparameters}

Following \citet{bosselut2019comet}, we use a dropout rate of 0.1 and GeLU \cite{hendrycks2020gaussian} units as activation functions. During training, we use the Adam optimizer \cite{kingma2017adam} with a batch size of 64. For COMET models trained on different subsets of the \atomic{} dataset, we adopt a maximum learning rate of 6.25e-5 with a warmup period of 0.002 times of the total number of minibatches customized for each model, which decays linearly until finishing training. We train different COMET models for different subsets of the full  on original data (\textbf{O}), original and logical negation data (\textbf{O+L}), original and semi-logical negation data (\textbf{O+S}), original and pragmatic negation data (\textbf{O+P}), and the overall dataset (\textbf{O+L+S+P}), for 21k, 25k, 24k, 24k and 29k minibatches respectively, and apply early stopping for all models. The rest of the hyperparameters are the same as those of GPT2-M in \citet{Radford2019LanguageMA} implemented via the publicly available HuggingFace API\footnote{https://huggingface.co/transformers/}.

\section{Negation Discriminator for Inconsistent Inferences}
\label{sec:model-discriminator}

The negation discriminator is designed to identify plausible generations of negated events. We fine-tune RoBERTa\textsubscript{BASE} \cite{liu2019roberta} as a binary classifier with automatically constructed logically valid and invalid commonsense knowledge triples in the \atomic{} form. 

\paragraph{Data}

The logically valid and invalid data used to train the negation discriminator is automatically constructed from the \atomic{} original and negation dataset. Positive training samples are comprised of the original and newly crowdsourced negation data from \atomic{}. To construct negative training samples, we leverage the concept of common and contrastive sets by swapping the set of contrastive differences between paired original and negation events. Specifically, we replace conditions of original events with distinct conditions of their negation counterparts and vice versa. For example, to construct a negative example of \textit{$\{$``PersonX passes the exam'', xNeed, ``to study hard''$\}$}, we replace the condition object with ``to miss classes all the time,'' which is a condition of the corresponding logical negation event ``PersonX does not pass the exam'' under the same relation. 

To balance the overall dataset, we sample the same proportion of positive and negative knowledge triples of original and negation events, respectively. Since the boundary between commonsense inferences of negated event pairs is not clear-cut, conditions in the human-annotated contrastive sets may fall into the common set as well, so not all training data has a golden label. However, previous work demonstrates that introducing a proper degree of noise improves the training outcome \cite{Luo2014DeepLW}.
The four versions of negation discriminators and their respective training data are shown in Table \ref{tab:discriminator-data-stats}.

\begin{table}
\small
% \renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{l|c|c}

\textbf{Discriminator} & \textbf{Data Subset} & \textbf{$\#$Trn} \\ 
\midrule

 Logical (L) & \dataset-L & 324,843 \\ 
 Semi-logical (S) & \dataset-S &  194,732 \\ 
 Pragmatics (P) & \dataset-P &  276,272 \\ 
%  Logical+Semi-logical (LS) & 519,574 \\
 All Negation Data (LSP) & \dataset & 795,845 \\
\bottomrule
\end{tabular}

\caption{Statistics of data used to train negation discriminators.} 
\label{tab:discriminator-data-stats}
\end{table}


\paragraph{Input}

As input to the discriminator model, we design sentence patterns that express relation types in natural language and fill out the patterned sentences with events and conditions before encoding them (e.g., ``PersonX addresses a talk. As a result, PersonX wants to convince others.''). Relations and their corresponding patterned sentences are listed in Table \ref{tab:discriminator-pattern} in Appendix \ref{sec:appendix}. Adopting patterned sentences is found to be a more effective approach than concatenating components in knowledge triples from the pilot study. 

\paragraph{Loss Function}

The negation discriminator is trained to minimized the binary cross-entropy loss for each example:

\begin{equation}
\mathcal{L}_{D} = y \cdot \log{P( y)} + (1-y) \cdot \log{(1-P( y))}
\label{eq:comet-loss}
\end{equation}

\noindent where $y$ is the label for an input (i.e., logically valid or invalid).
 
\paragraph{Hyperparameters}

Parameters are initialized with the trained weights of the RoBERTa-base model in \citet{liu2019roberta}. %with 24 layers, 768-dimensional hidden states and 12 attention heads. 
During training, we use the Adam optimizer \cite{kingma2017adam} and train the model with a batch size of 64. We adopt a maximum learning rate of 4.5e-5 with a warmup period of 10 minibatches. We trained \textbf{L}, \textbf{S}, \textbf{P}, \textbf{LSP}, for 25K, 14K, 21K and 6K minibatches respectively, and apply early stopping for all models. We use a probability threshold of 0.7 to determine whether an input knowledge triple to the discriminator is plausible based on pilot study on the development sets. The rest of the hyperparameters are the same as those of RoBERTa-base \cite{liu2019roberta} implemented via the publicly available HuggingFace API\footnote{https://huggingface.co/transformers/}.


==> sections/Z5-experiment-Old.tex <==
\section{Experiment}
\label{sec:exps}

We evaluate two methods of improving COMET's ability of predicting around events with negation cues: fine-tuning COMET on negation data or/and applying logic discriminators to separate logically valid and invalid generations. 

\subsection{COMET with Negation Data}
\label{sec:exp-comet-neg-data}

\paragraph{Baselines}

As described in Section \ref{sec:model-comet}, we combine ATOMIC original with logical negation (\textbf{O+Ln}), semi-logical negation (\textbf{O+Sn}) and both logical and semi-logical negation data (\textbf{O+Ln+Sn}) for training COMET. As a baseline, we also train COMET only on the original data (\textbf{O}).

\paragraph{Metrics}

Following \citet{bosselut2019comet}, we evaluate the quality of COMET generations with BLEU-2\cite{bleu-2003} as an automatic evaluation metric. We also include the perplexity of models on their reference generations. 

For the human evaluation, we employ human judges from Amazon Mechanical Turk (AMT) to identify whether generated ATOMIC commonsense conditions given events and typed relations of various COMET models are adequately plausible. 
We compiled a list of original events from the ATOMIC original test set with both their logical and semi-logical negation counterparts included in their test set.
We randomly sampled 100 such original events with corresponding logical and semi-logical events to conduct human evaluation. 

Following  \citet{bosselut2019comet} and \citet{sap2019atomic}, for each event and relation type, 10 options of the inferred condition are generated with beam search. We present the full beam to five distinct crowdworkers and ask them to select all plausible options. For each model (\textbf{O}, \textbf{O+Ln}, \textbf{O+Sn}, \textbf{O+Ln+Sn}), 45K annotations are collected for each of the original, logical negation and semi-logical negation test sets (100 events $\times$ 9 relations $\times$ 10 options $\times$ 5 annotations), resulting in 135K annotations per model. We calculate the average precision at 10 (P@10), the average number of correct generations per dimension, for generations of each model across different evaluation sets. The full assessment of different versions of COMET models is reported in Table \ref{tab:comet-neg-auto-eval}.

% \begin{table}
% \small
% \renewcommand{\arraystretch}{1.1}
% \centering
% \begin{tabular}{l|lrrrr}

%  \textbf{Eval Set} & \textbf{Trn Set} & \textbf{PPL $\downarrow$} & \textbf{BLEU $\uparrow$} & \textbf{P@10 $\uparrow$} \\ 
%  \midrule

%  \multirow{4}{*}{original} & O & 9.30 & 14.18 & 53.22 \\
%  & O+Ln & \textbf{9.27} & \textbf{14.20} & \textbf{55.60} \\ 
%  & O+Sn & 9.30 & 14.09 & 48.35 \\ 
%  & O+Ln+Sn & 9.29 & 14.12 & 49.40 \\  
%  \midrule
 
%  \multirow{4}{*}{\makecell[tl]{logical}} & O & 10.87 & 10.86 & 33.21 \\ 
%  & O+Ln & 9.28 & 11.94 & \textbf{46.69} \\ 
%  & O+Sn & 9.93 & 11.29 & 40.18 \\ 
%  & O+Ln+Sn & \textbf{9.17} & \textbf{12.00} & 41.51 \\ 
%  \midrule
 
%  \multirow{4}{*}{\makecell[tl]{semi}}& O & 11.69 & 12.07 & 35.15 \\ 
%  & O+Ln & 10.69 & 12.69 & \textbf{42.13} \\ 
%  & O+Sn & 10.23 & 12.79 & 41.75 \\
%  & O+Ln+Sn & \textbf{9.93} & \textbf{13.23} & 35.68 \\ 
%  \midrule
 
%  \multirow{4}{*}{\makecell[tl]{logical\\+semi}}& O & 11.19 & 11.30 & - \\ 
%  & O+Ln & 9.82 & 12.20 & - \\ 
%  & O+Sn & 10.05 & 11.84 & - \\ 
%  & O+Ln+Sn & \textbf{9.46} & \textbf{12.45} & - \\ 
%  \bottomrule

% \hline
% \end{tabular}
% \caption{Evaluations of COMET models trained on different combinations of the original and negation ATOMIC data.}
% \label{tab:comet-neg-auto-eval}
% \end{table}

\begin{table}
\small
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l|lrrrr}

 \textbf{Eval} & \textbf{Trn Set} & \textbf{PPL $\downarrow$} & \textbf{BLEU $\uparrow$} & \textbf{P@10 $\uparrow$} \\ 
 \midrule

 \multirow{4}{*}{original} & O & 9.30 & 14.18 & 53.22 \\
 & O+L & \textbf{9.27} & \textbf{14.20} & \textbf{55.60} \\ 
 & O+S & 9.30 & 14.09 & 48.35 \\ 
 & O+P & 9.29 &  & 52.16 \\ 
 & O+L+S & 9.29 & 14.12 & 49.40 \\  
 & O+L+S+P & 9.28 &  & 51.94 \\  
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{logical}} & O & 10.87 & 10.86 & 33.21 \\ 
 & O+L & 9.28 & 11.94 & 46.69 \\ 
 & O+S & 9.93 & 11.29 & 40.18 \\ 
 & O+P & 10.34 &  & 43.18 \\ 
 & O+L+S & 9.17 & 12.00 & 41.51 \\ 
 & O+L+S+P & \textbf{9.08} &  & \textbf{51.55} \\ 
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{semi}}& O & 11.69 & 12.07 & 35.15 \\ 
 & O+L & 10.69 & 12.69 & 42.13 \\ 
 & O+S & 10.23 & 12.79 & 41.75 \\
 & O+P & 10.95 &  & 45.84 \\ 
 & O+L+S & 9.93 & 13.23 & 35.68 \\ 
 & O+L+S+P & \textbf{9.80} &  & \textbf{53.02} \\ 
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{prag}} & O & 12.02 &  & 52.12 \\ 
 & O+L & 11.72 &  & \textbf{53.16} \\ 
 & O+S & 11.67 &  & 49.84 \\ 
 & O+P & 11.50 &  & 37.41 \\ 
 & O+L+S & 11.48 &  & 48.15 \\ 
 & O+L+S+P & \textbf{11.20} &  & 41.53 \\ 
 \bottomrule

\hline
\end{tabular}
\caption{Evaluations of COMET models trained on different combinations of the original and negation ATOMIC data.}
\label{tab:comet-neg-auto-eval}
\end{table}

\paragraph{Results}

While the original COMET model is capable of producing correct generations with P@10 of 53.22, it generates less plausible predictions for the logical and semi-logical negation events, with P@10 of 33.21 and 35.15 respectively. However, by adding either or both types of negation events into the training data, COMET is able to make better predictions about both logical and semi-logical negation events. Note that although COMET with \textbf{O+Ln} does not have the best automatic scores with respect to negation evaluation sets, it produces generation with the highest quality by increasing P@10 over baselines by 40.6\% and 19.9\% for logical and semi-logical negation respectively. Whereas \textbf{O+Ln+Sn}, which has the lowest perplexity and highest BLEU-2 scores over negation evaluation sets, achieves poorer-quality generations reflected by lower P@10. Such discrepancy is a reaffirmation of the observation that automatic metrics have limited ability of representing the overall quality of generative language models.

It is also noticeable that training on logical negation also increases P@10 for the semi-logical negation, and vice versa, indicating that COMET successfully distill knowledge from logical and semi-logical negation data and can transfer the learning outcomes between negation types. However, when combining logical with semi-logical negation in \textbf{O+Ln+Sn}, the learning outcomes do not transfer well over neither negation type. 


\subsection{Discriminator}

\begin{table}
% \small
\footnotesize
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{4.5pt}
\centering
\begin{tabular}{l|l|ccc|ccc}
 
%  \toprule
 \multicolumn{2}{l|}{} & \multicolumn{3}{c|}{\textbf{BLEU-2}} & \multicolumn{3}{c}{\textbf{HE}}  \\ 
 \midrule
 
 \multicolumn{2}{c|}{\diagbox[width=\widthof{xxxxxxxxxx}]{\textbf{Eval}}{\textbf{Dis}}} & \textbf{L} & \textbf{S} & \textbf{LS} & \textbf{L} & \textbf{S} & \textbf{LS} \\ 
 \midrule

 \multirowcell{3}{O} & all & 14.18 & \textbf{14.18} & 14.18 & 53.22 & 53.22 & 53.22\\
 & vld & \textbf{14.21} & \textbf{14.18} & \textbf{14.25} & \textbf{53.70} & \textbf{54.18} & \textbf{54.26} \\ 
 & inv & 12.75 & 13.81 & 12.56 & 42.62 & 43.13 & 41.12 \\ 
 \midrule
 
 \multirowcell{3}{Ln} & all & 10.86 & 10.86 & 10.86 & 33.21 & 33.21 & 33.21 \\ 
 & vld & \textbf{11.44} & \textbf{11.26} & \textbf{11.26} & \textbf{44.61} & \textbf{40.71} & \textbf{44.54} \\ 
 & inv & 10.03 & 10.17 & 10.11 & 23.97 & 23.69 & 24.04 \\ 
 \midrule
 
 \multirowcell{3}{Sn} & all & 12.07 & 12.07 & 12.07 & 35.15 & 35.15 & 35.15 \\
 & vld & \textbf{12.12} & \textbf{12.48} & \textbf{12.33} & \textbf{35.62} & \textbf{44.91} & \textbf{45.28} \\ 
 & inv & 11.26 & 11.45 & 11.41 & 25.99 & 27.42 & 27.12 \\ 
 \midrule
 
 \multirowcell{3}{Ln\\+Sn} & all & 11.30 & 11.30 & 11.30 & - & - & - \\
 & vld & \textbf{11.87} & \textbf{11.69} & \textbf{11.67} & - & - & - \\ 
 & inv & 10.12 & 10.64 & 10.56 & - & - & - \\ 
 \bottomrule
 
\end{tabular}

\caption{Average BLEU-2 scores of beam search generations of the COMET model trained on ATOMIC original over various evaluation sets, classified into \textit{valid} and \textit{invalid} sets by discriminators.}
\label{tab:comet-disc-bleu2}
\end{table}


\begin{table}
\small
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l|l|lll}

 \toprule
 \multicolumn{2}{l|}{\diagbox[width=\widthof{xxxxxxxxxxxxxxxx}]{\textbf{Eval}}{\textbf{Disc}}} & \textbf{LD} & \textbf{SD} & \textbf{LSD} \\ 
 \midrule

 \multirowcell{3}{original} & all & \textbf{61.95} & \textbf{64.44} & \textbf{63.08} \\
 & valid & 61.71 & 63.91 & 62.90 \\ 
 & invalid & 50.50 & 53.60 & 54.49 \\ 
 \midrule
 
 \multirowcell{3}{logical} & all & 42.64 & 41.84 & 41.72 \\ 
 & valid & \textbf{51.97*} & \textbf{46.70*} & \textbf{49.78*} \\ 
 & invalid & 30.46 & 30.90 & 28.74 \\ 
 \midrule
 
 \multirowcell{3}{semi} & all & 41.21 & 42.13 & 39.32 \\
 & valid  & \textbf{48.30*} & \textbf{48.33*} & \textbf{46.07*} \\ 
 & invalid & 29.30 & 33.57 & 27.70 \\ 
 \midrule
 
\end{tabular}
\caption{Precision at 3 (\textit{P@3}) for the \textit{all}, \textit{valid} and \textit{invalid} sets obtained by applying discriminators to generations of the COMET model trained on ATOMIC original across three evaluation sets. Every \textit{valid} and \textit{all} sets outperform the corresponding \textit{invalid} set significantly at $p < 0.01$. Asterisks mark \textit{valid} sets that outperform their corresponding \textit{all} set at $p < 0.01$.}
\label{tab:rerank-human-eval}
\end{table}



\begin{table}
% \footnotesize
\small
\centering
\begin{tabular}{l|l|lc}

\toprule
\textbf{Event + Rel} & \textbf{Generation} & \textbf{V} & \textbf{C}\\
\midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not skate \\around\\\textbf{\textbf{xAttr}}}} & athletic & \xmark & \cmark \\
 & careless & \xmark & \cmark \\
 & lazy & \cmark & \cmark \\
 & uncoordinated & \cmark & \cmark \\
 & unskilled & \cmark & \cmark \\ 
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not sit \\behind Y\\\textbf{\textbf{xIntent}}}} & to be alone & \cmark & \cmark \\
 & to be left alone & \cmark & \cmark \\
 & to avoid Y & \cmark & \cmark \\
 & to sit & \xmark & \cmark \\
 & to wait & \cmark & \cmark \\
 \midrule

 \multirow{5}{*}{\makecell[tl]{X does \\not look \\angry\\\textbf{\textit{xNeed}}}} & to calm down & \cmark & \cmark \\
 & to watch a movie & \xmark & \cmark \\
 & to have been provoked & \xmark & \cmark \\
 & to not be angry & \xmark & \xmark \\
 & to be calm & \cmark & \cmark \\
 \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X does \\not rent \\an apartment\\\textbf{\textit{xWant}}}} & to save money & \cmark & \cmark \\
%  & to get a job & \cmark & \cmark \\
%  & to pay rent & \xmark & \cmark \\
%  & to move in & \xmark & \cmark \\
%  & to get a new apartment & \xmark & \cmark \\
%  \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X is \\not offered \\the job\\\textbf{\textit{oWant}}}} & to hire X & \xmark & \xmark \\
%  & to fire X & \cmark & \cmark \\
%  & to hire someone else & \cmark & \cmark \\
%  & to accept the job & \xmark & \cmark \\
%  & to hire them & \xmark & \cmark \\
%  \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X does\\not buy \\a snack\\\textbf{\textit{xReact}}}} & satisfied & \xmark & \cmark\\
%  & hungry & \cmark & \cmark\\
%  & satiated & \xmark & \cmark\\
%  & full & \xmark & \cmark\\
%  & guilty & \cmark & \cmark\\
%  \midrule
 
 \multirow{5}{*}{\makecell[tl]{X refuses \\to hear a \\scary noise\\\textbf{\textit{xWant}}}} & to run away & \xmark & \xmark \\
 & to go to sleep & \cmark & \cmark \\
 & to be safe & \cmark & \cmark \\
 & to keep quiet & \cmark & \cmark \\
 & to avoid the noise & \cmark & \cmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X never \\brings Y into \\conflicts\\\textbf{\textit{oWant}}}} & to avoid X & \xmark & \xmark \\
 & to be left alone & \xmark & \cmark \\
 & to thank X & \cmark & \cmark \\
 & to fight back & \xmark & \xmark \\
 & to avoid conflict & \xmark & \cmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X scarcely\\gets sunburned\\ \\\textbf{\textit{xReact}}}} & burned & \xmark & \xmark\\
 & hurt & \xmark & \xmark\\
 & sick & \xmark & \xmark\\
 & sad & \xmark & \xmark\\
 & satisfied & \cmark & \cmark\\
 \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X does \\not bring Y\\into conflict\\\textbf{\textit{oWant}}}} & relieved & \cmark & \cmark \\
%  & sad & \xmark & \cmark \\
%  & satisfied & \cmark & \cmark \\
%  & grateful & \cmark & \cmark \\
%  & angry & \xmark & \cmark \\
%  \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X does \\not learn \\new things\\\textbf{\textit{xEffect}}}} & gains knowledge & \xmark & \cmark \\
%  & becomes lazy & \cmark & \cmark \\
%  & gets bored & \cmark & \cmark \\
%  & becomes ignorant & \cmark & \cmark \\
%  & cries & \cmark & \cmark \\
%  \midrule
 
%  \multirow{5}{*}{\makecell[tl]{X does \\not put Y \\in mind\\\textbf{\textit{oEffect}}}} & becomes confused & \xmark & \cmark \\
%  & does not think about X & \cmark & \cmark \\
%  & Y thinks about X & \xmark & \cmark \\
%  & Y is not remembered & \cmark & \cmark \\
%  & cries & \xmark & \xmark \\
% \bottomrule

\end{tabular}
\caption{Randomly selected generations from the \textbf{ATOMIC logical negation} set. The top 5 options are classified as either \textit{valid} or \textit{invalid} by the \textbf{logical+semi discriminator}. \textbf{V} indicates whether the generation is classified as \textit{valid} by the discriminator. \textbf{C} indicates whether options are correctly classified by human judges.} 
\label{tab:discriminator-generations-logical}
\end{table}


\begin{table*}
\small
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l|l|rrr|rrr|rrr}

 \multicolumn{2}{l|}{Discriminator} & \multicolumn{3}{c|}{\textbf{Logical}} & \multicolumn{3}{c|}{\textbf{Semi}} & \multicolumn{3}{c}{\textbf{\textbf{Logical+Semi}}} \\ 
 \midrule

 \multicolumn{2}{l|}{Eval Set} & \multicolumn{1}{r}{\textbf{Prec}} & \multicolumn{1}{r}{\textbf{Rec}} & \multicolumn{1}{r|}{\textbf{F1}} & \multicolumn{1}{r}{\textbf{Prec}} & \multicolumn{1}{r}{\textbf{Rec}} & \multicolumn{1}{r|}{\textbf{F1}} & \multicolumn{1}{r}{\textbf{Prec}} & \multicolumn{1}{r}{\textbf{Rec}} & \multicolumn{1}{r}{\textbf{F1}} \\ 
 \midrule
 
 \multirowcell{2}{O} & valid & 53.70 & 96.53 & 69.01 & 54.18 & 92.91 & 68.45 & 54.26 & 93.87 & 68.77 \\
 & invalid & 57.38 & 5.32 & 9.73 & 56.87 & 10.63 & 17.91 & 58.88 & 9.98 & 17.07 \\
 \midrule
 
 \multirowcell{2}{Ln} & valid & 44.61 & 60.11 & 51.22 & 40.71 & 68.56 & 51.09 & 44.54 & 59.98 & 51.12 \\
 & invalid & 76.03 & 62.90 & 68.84 & 76.31 & 50.36 & 60.68 & 75.96 & 62.87 & 68.80 \\
 \midrule

 \multirowcell{2}{Sn} & valid & 35.62 & 96.43 & 52.02 & 44.91 & 56.48 & 50.03 & 45.28 & 56.97 & 50.46 \\
 & invalid & 74.01 & 5.50 & 10.24 & 72.58 & 62.44 & 67.13 & 72.88 & 62.69 & 67.40 \\
 \midrule
 
\end{tabular}
\caption{Precision, recall and F1 scores for the \textit{valid} and \textit{invalid} sets of applying various discriminators to the generations of the COMET model trained on ATOMIC original.}
\label{tab:partition-f1}
\end{table*}

\paragraph{Baselines}

As described in Section \ref{sec:model-discriminator}, we fine-tune RoBERTa\textsubscript{BASE} with logical negation, semi-logical negation and the combination of both to obtained three negation discriminators (i.e., \textbf{L}, \textbf{S}, \textbf{LS}). By applying a negation discriminator to a set of candidates generated by COMET, it classifies each option as either logically \textit{valid} or \textit{invalid}, partitioning the overall set of candidates into \textit{valid} and \textit{invalid} sets. We employ COMET generations without applying discriminators (i.e., the \textit{all} set) as baselines. 
 
\paragraph{Metrics}

We evaluate and compare the quality of the \textit{all}, \textit{valid} and \textit{invalid} sets automatically with BLEU-2 and with accuracy, precision, recall and F1 scores based on the human evaluation. 

To assess the quality of a discriminator, we use the same human evaluation scores as in Section \ref{sec:exp-comet-neg-data} but calculate accuracies (i.e., the percentage of correct options among all candidates) separately for each of the \textit{all}, \textit{valid} and the \textit{invalid} sets. The \textit{all} set contains the full beam with 10 elements, while the \textit{valid} and \textit{invalid} sets have varying number of elements depending on how discriminators classify them, summing to 10. In addition, for each evaluation set and applied each discriminator, per relation, we randomly selected a subset of 25 events that have at least three options in both the \textit{valid} and \textit{invalid} sets and compare their P@3, calculated as the percentage of correct options among top three options. We also report the precision, recall and F1 scores for the \textit{valid} and \textit{invalid} set to assess discriminators' ability of identifying logic flaws in commonsense reasoning.

Finally, while by applying the discriminator to the full beam we get a \textit{valid} subset with higher accuracy, we have less correct options in total. Thus we also investigate the efficiency of using discriminators to expand the commonsense KB. We use the COMET model to generate beams with size 25 and then apply the discriminator to the full beam. We collect human annotations for the same 100 events but with generations of beam size of 25. We compare the number of correct candidates and the accuracy of the \textit{valid} set of beam 25 to the \textit{all} set of beam 10 in Table \ref{tab:valid-option-yield}.

\paragraph{Results}
% \paragraph{Results}
The BLEU-2 and human evaluation accuracy scores in Table \ref{tab:comet-disc-bleu2} demonstrate that all types of negation discriminators (\textbf{L}, \textbf{S} and \textbf{LS}) are able to extract a subset of candidates with higher average quality than the set directly generated by the COMET model, for both negation and original events. While discriminators trained only on logical or semi-logical negation are specialized in their corresponding type of data, they also achieve higher percentage accuracy for the \textit{valid} set of other types of negation and the original data in small margins, demonstrates a transferred learning outcome.
Particularly, the discriminator trained on both logical and semi-logical negations improves the accuracy of logical and semi-logical negation typed generations by 34.1\% and 28.8\% respectively in Table \ref{tab:comet-disc-bleu2}. 
In Table \ref{tab:partition-f1}, recall scores indicate that around 62\% of the incorrect candidates from the full beam are successfully ruled out, while about 60\% correct candidates are selected by the logical and semi-logical discriminator for both the logical and semi-logical evaluation sets.
Table \ref{tab:discriminator-generations-logical} shows examples of \textit{valid} and \textit{invalid} candidates for logical negation events as specified by the logical and semi-logical discriminator.

When we restrict examples to prompts with at least three elements in both the \textit{valid} and \textit{invalid} set, the top three elements in the \textit{valid} set significantly outperforms the top three options from the original beam at $p < 0.01$ for all negation discriminators and across both logical and semi-logical evaluation sets. However, for original events, such improvement does not hold. This indicates that if a query event is known to be in the negation form, then we can apply the discriminators as an reranking mechanism towards the original beam to remove options that are less plausible to get better candidate sets.

\begin{table}
\small
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l|lll}

 \multicolumn{1}{l|}{Eval}  & \multicolumn{1}{c}{\textbf{O}} & \multicolumn{1}{c}{\textbf{Ln}} & \multicolumn{1}{c}{\textbf{Sn}} \\ 
 \midrule
 baseline & 53.22 & 33.21 & 35.15 \\
 \midrule
 all & 55.60 & 46.69 & 42.13 \\
 valid & \textbf{56.45} & \textbf{54.82} & \textbf{51.02} \\ 
 invalid & 45.78 & 33.48 & 31.75 \\ 
 
\end{tabular}
\caption{Human evaluation scores for applying the \textbf{LS} discriminators to beam search generations of COMET trained on \textbf{O+Ln}. \textbf{Bold} numbers indicate the set with the highest score among \textit{all}, \textit{valid} and \textit{invalid} sets.}
\label{tab:comet-ol-dis-ls-human-eval}
\end{table}

Furthermore, we apply negation discriminators to the COMET model trained on negation data and achieve further improvement over the quality of the select output set. Table \ref{tab:comet-ol-dis-ls-human-eval} shows that by applying the \textit{LS} discriminator to generations of the \textit{O+Ln} version of COMET model, the accuracy score of valid set gains 6\%, 65\% and 45\% reletive improvement over the original, logical and semi-logical negations baseline sets respectively, which are the raw beams of the COMET trained on \textit{O}.

\begin{table*}
\small
% \footnotesize
\renewcommand{\arraystretch}{0.8}
\centering
\begin{tabular}{l|l|rrr|rrr|rrr}

\multicolumn{2}{l|}{\textbf{Evaluation Set}} & \multicolumn{3}{c|}{\textbf{Original}} & \multicolumn{3}{c|}{\textbf{Logical}} & \multicolumn{3}{c}{\textbf{\textbf{Semi}}}  \\ 
\midrule

 \textbf{Beam} & \textbf{Set} & \textbf{$\#$\cmark} & \textbf{$\#$total} & \textbf{$\%$\cmark} & \textbf{$\#$\cmark} & \textbf{$\#$total} & \textbf{$\%$\cmark} & \textbf{$\#$\cmark} & \textbf{$\#$total} & \textbf{$\%$\cmark} \\
 \midrule
 
 
  \multirow{2}{*}{\textbf{10}} & all & 5.32 & 10.00 & 53.22 & 3.32 & 10.00 & 33.21 & 3.52 & 10.00 & 35.15 \\
 & valid & 5.00 & 9.21 & 54.26 & 1.99 & 4.47 & 44.54 & 2.00 & 4.42 & 45.28 \\ 
 \cmidrule{0-1}
 
 \multirow{2}{*}{\textbf{25}} & all & 12.24 & 25.00 & 48.98 & 7.86 & 25.00 & 31.44 & 7.45 & 25.00 & 29.78 \\
 & valid & 11.35 & 22.86 & 49.65 & \textbf{4.20} & 10.69 & \textbf{39.29} & \textbf{4.04} & 10.98 & \textbf{36.77} \\ 
 \bottomrule

\end{tabular}

\caption{Yields of correct generations of applying the logical+semi discriminator (\textbf{LSD}) to generations of COMET trained on ATOMIC original for beam size of 10 and 25. \textit{$\#$\cmark} is the number of correct options yielded. \textit{$\#$total} is the total number of options in each set. \textit{$\%$\cmark} is the percentage correctness.}
\label{tab:valid-option-yield}
\end{table*}

Finally, for the efficiency of using discriminators to expand the commonsense KB, Table \ref{tab:valid-option-yield} shows that for both logical and semi-logical types, the \textit{valid} set of beam 25 has higher accuracy and more correct options than the \textit{all} set of beam 10. This indicates that when we have a larger and potentially more noisy set of candidates, by applying the negation discriminator, we are able to get a set of options that have both higher quality and higher correct option yields than using the full beam with smaller beam size of 10.

==> sections/Z5-experiment.tex <==
\section{Experiments}
\label{sec:exps}

We evaluate two methods of improving COMET's ability of predicting around negation events: fine-tuning COMET on negation data or/and applying negation discriminators to filter out generations that are logically plausible. 

\subsection{COMET with Negation Data}
\label{sec:exp-comet-neg-data}

\begin{table}
\small
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{l|lrrrr}

 \textbf{Eval} & \textbf{Trn Set} & \textbf{PPL $\downarrow$} & \textbf{B2 $\uparrow$} & \textbf{P@10 $\uparrow$} \\ 
 \midrule

 \multirow{2}{*}{\atomic} & \atomic & 9.30 & \textbf{14.18} & \textbf{55.18} \\
 & \atomic{} + \dataset{} & \textbf{9.28} & 14.05 & 53.61 \\  
 \midrule
 
 \multirow{2}{*}{\makecell[tl]{\dataset-L}} & \atomic & 10.87 & 10.86 & 35.84 \\ 
 & \atomic{} + \dataset{} & \textbf{9.08} & \textbf{11.96} & \textbf{45.42} \\ 
 \midrule
 
 \multirow{2}{*}{\makecell[tl]{\dataset-S}}& \atomic & 11.69 & 12.07 & 36.89 \\ 
 & \atomic{} + \dataset{} & \textbf{9.80} & \textbf{13.22} & \textbf{46.88} \\ 
 \midrule
 
 \multirow{2}{*}{\makecell[tl]{\dataset-P}} & \atomic & 12.02 & 14.32 & 46.70 \\ 
 & \atomic{} + \dataset{} & \textbf{11.20} & \textbf{14.64} & \textbf{50.65} \\ 
 \bottomrule

\hline
\end{tabular}
}
\caption{Evaluations of COMET models trained on different combinations of the \atomic{} and \dataset{} knowledge graphs. Training on examples of negated events leads to large improvements in the quality of generated inferences with minimal dropoff in the quality of inferences for positive polarity events.}
\label{tab:comet-neg-result-main}
\end{table}


\paragraph{Data and baseline}

We first train COMET on the overall \atomic{} data, including the original, logical negation, semi-logical negation, and pragmatic negation data (\textbf{O+L+S+P}) to expand the commonsense KB along both affirmative and negated dimensions. The combined dataset is shuffled so that the original and negation data are uniformly mixed during training and evaluation. As a baseline, we also train COMET solely on the original data (\textbf{O}). As an ablation study, we trained COMET on both the original and logical negation data (\textbf{O+L}), the original and semi-logical negation data (\textbf{O+S}), and the original and pragmatic negation data (\textbf{O+P}).


\paragraph{Metrics}

Following \citet{bosselut2019comet}, we evaluate the quality of COMET generations with BLEU-2\cite{bleu-2003} as an automatic evaluation metric. We also include the perplexity of models on their reference generations. 

For the human evaluation, we employ human judges from MTurk to identify whether generated \atomic{} commonsense conditions given events and typed relations of various COMET models are adequately plausible. 
We compiled a list of original events from the \atomic{} original test set with their logical, semi-logical, and pragmatic negation counterparts included in their test sets.
We randomly sampled 100 such original events with corresponding logical, semi-logical, and pragmatic negation events to conduct the human evaluation. 

Following  \citet{bosselut2019comet} and \citet{sap2019atomic}, for each event and relation type, 10 options are generated with beam search. We present the full beam of each event-relation prompt to at least six distinct crowdworkers and ask them to select all plausible options. We conduct comprehensive pre- and post-evaluation screening on the users and the tasks being completed to ensure the objectivity and high quality of the evaluations. Besides qualifying users before tasks, we double check to remove evaluation tasks that are not carefully conducted (e.g., tasks done by users that select all/no options for all hundreds of tasks that they perform, etc.). To ensure comparable evaluation sets with a balanced number of examples under each prompt across models, we randomly sample at most five evaluations from the screened evaluation set for each event-relation prompt. For each model (\textbf{O}, \textbf{O+Ln}, \textbf{O+S}, \textbf{O+P}, \textbf{O+L+S+P}) with respect to each evaluation set (\textbf{O}, \textbf{L}, \textbf{S}, \textbf{P}), at most 45K (m=43,374, $\sigma$=1,848) annotations are used to compute the final human evaluation score (100 events $\times$ 9 relations $\times$ 10 options $\times$ at most 5 annotations). 

We calculate the average precision at 10 (P@10), the average number of correct options per event-relation prompt, for each model's generations across different evaluation sets. The full assessment of COMET model trained on \atomic{} original and negation data is reported in Table \ref{tab:comet-neg-result-main} and the ablation result is reported in Table \ref{tab:comet-neg-result-ablation}.

\begin{table}
\small
% \renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l|lrrrr}

 \textbf{Eval} & \textbf{Trn Set} & \textbf{PPL $\downarrow$} & \textbf{BLEU $\uparrow$} & \textbf{P@10 $\uparrow$} \\ 
 \midrule

 \multirow{4}{*}{\atomic} & \atomic & 9.30 & 14.18 & 55.18 \\
 & + \dataset-L & \textbf{9.27} & \textbf{14.20} & \textbf{58.11} \\ 
 & + \dataset-S & 9.30 & 14.09 & 55.74 \\ 
 & + \dataset-P & 9.29 & 14.10 & 52.22 \\ 
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{\dataset-L}} & \atomic & 10.87 & 10.86 & 35.84 \\ 
 & + \dataset-L & \textbf{9.28} & \textbf{11.94} & \textbf{44.94} \\ 
 & + \dataset-S & 9.93 & 11.29 & 44.01 \\ 
 & + \dataset-P & 10.34 & 11.04 & 42.33 \\ 
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{\dataset-S}}& \atomic & 11.69 & 12.07 & 36.89 \\ 
 & + \dataset-L & 10.69 & 12.69 & 42.38 \\ 
 & + \dataset-S & \textbf{10.23} & \textbf{12.79} & \textbf{45.50} \\
 & + \dataset-P & 10.95 & 12.35 & 41.76 \\ 
 \midrule
 
 \multirow{4}{*}{\makecell[tl]{\dataset-P}} & \atomic & 12.02 & 14.32 & 46.70 \\ 
 & + \dataset-L & 11.72 & 14.43 & 47.78 \\ 
 & + \dataset-S & 11.67 & 14.34 & 46.09 \\ 
 & + \dataset-P & \textbf{11.50} & \textbf{14.58} & \textbf{48.79} \\ 
 \bottomrule

\hline
\end{tabular}
\caption{Ablation results of knowledge models trained and evaluated on different portions of the \dataset{} knowledge graph of negated events. The best result on each subset of \dataset{} comes from training on similar examples. The model trained on negated events from \dataset-L performs the best at generating inferences for the original \atomic{} events.}
\label{tab:comet-neg-result-ablation}
\end{table}



\paragraph{Results}

While the original COMET model can produce correct generations with P@10 of 55.18 for the original \atomic{} test set, its performance regarding logical and semi-logical negation events drops substantially for approximately 35\%, with 33.84 and 36.89 P@10 respectively. Although pragmatic negation events share similar sentence structures as original events without specific negation cues, since they are human crafted, they tend to be more creative and diverse than the corpora extracted events as in the original \atomic{} dataset. Therefore, the performance over pragmatic negation events also experiences a 9.6\% drop from the original task. 

By training COMET on both the original and negation data (\textbf{O+L+S+P}), as shown in Table \ref{tab:comet-neg-result-main}, COMET's performance increases over logical negation events for 26.7\%, semi-logical events for 27.1\%, and pragmatic negation events for 8.5\%, while maintains the approximately same level of performance over the original events under human evaluation. The BLEU-2 scores share similar trends as human evaluation scores, indicating that the newly proposed \atomic{} negation data effectively improves COMET's ability to make commonsense inferences over negated events reflected by both human and automatic evaluation metrics.

When we separate the effects of different negation types, Table \ref{tab:comet-neg-result-ablation} shows that while each negation type improves COMET's performance most effectively with respect to their own type of data, they can transfer the learning outcomes between negation types as well. 
Notably, for COMET trained on \textbf{O+L}, it approaches a similar level of a performance boost as COMET trained on \textbf{O+L+S+P} across all negation types. 
Besides, it slightly improves over the original events as well, which is not observed from COMET trained on \textbf{O+L+S+P}. 
Such improvements across original and different negation types of events indicate that as simple as raising the model's awareness of the negation cue ``not'' results in some complex reasoning path involving negation, which boosts the model's commonsense reasoning ability overall.

\subsection{Negation Discriminator}

\paragraph{Baselines}

As described in Section \ref{sec:model-discriminator}, we fine-tune RoBERTa\textsubscript{BASE} with automatically constructed positive and negative data derived from logical negation, semi-logical negation, pragmatic negation and the combination of all to obtained four negation discriminators (i.e., \textbf{L}, \textbf{S}, \textbf{LP} and \textbf{LSP}). By applying a negation discriminator to a set of candidates generated by COMET, it classifies each option as either logically \textit{valid} or \textit{invalid}, partitioning the overall set of candidates into \textit{valid} and \textit{invalid} sets. We employ COMET generations without applying discriminators (i.e., the \textit{all} set) as baselines. 
 
\paragraph{Metrics}

We evaluate and compare the quality of the \textit{all}, \textit{valid} and \textit{invalid} sets automatically with BLEU-2 and with accuracy, precision, recall and F1 scores based on human evaluation scores. 

To assess the quality of a discriminator, we use the same human evaluation scores as in Section \ref{sec:exp-comet-neg-data} but calculate accuracies (i.e., the percentage of correct options among all candidates) separately for each of the \textit{all}, \textit{valid} and the \textit{invalid} sets. The \textit{all} set contains the full beam with 10 elements, while the \textit{valid} and \textit{invalid} sets have varying number of elements depending on how discriminators classify them, summing to 10. We also report the precision, recall and F1 scores for the \textit{all}, \textit{valid} and \textit{invalid} set to assess the negation discriminator's ability of identifying logic flaws in commonsense reasoning.

In addition, when we compare the \textit{valid} set to the full beam, since there are a different number of options in each set, it is not immediately obvious whether the \textit{valid} set is actually a better subset of the full beam than directly extracting the same number of elements from the top of the beam.
Therefore, we compute precision at the length of the valid set for the full beam, P@len(valid), by taking the same number of options as in the \textit{valid} set from the top of the ranked \textit{all} set, and calculate the accuracy of this subset. 
To compare P@len(valid) for the \textit{all} and \textit{valid} sets, we use Permutation Test\footnote{http://rasbt.github.io/mlxtend/} with 100k permutations to test for statistical significance. 

% In addition, we compute precision at the length of the valid set for the full beam, P@len(valid), by taking the same number of options as in the \textit{valid} set from the top of the \textit{all} set, and calculate the accuracy of this subset. 
% http://rasbt.github.io/mlxtend/user\_guide/evaluate/permutation\_test/

\paragraph{Results}

\begin{table}
\small
% \footnotesize
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{4.5pt}
\centering
\begin{tabular}{l|lrr|rrr}
 \textbf{Eval Set} & & \textbf{BL2$\uparrow$} & \textbf{Acc$\uparrow$} & \textbf{Prec$\uparrow$} & \textbf{Rec$\uparrow$} & \textbf{F1$\uparrow$} \\ 
 \midrule

 \multirowcell{3}{\atomic} & all & 14.18 & 55.18 & - & 1.00 & - \\
 & valid & \textbf{14.24} & \textbf{59.66} & 59.66 & 67.73 & 63.44 \\ 
 & invalid & 13.93 & 47.67 & 52.33 & 43.61 & 47.57 \\ 
 \midrule
 
 \multirowcell{3}{\dataset-L} & all & 10.86 & 35.84 & - & 1.00 & - \\ 
 & valid & \textbf{11.33} & \textbf{47.98} & 47.98 & 58.90 & 52.88 \\ 
 & invalid & 10.13 & 26.30 & 73.70 & 64.33 & 68.70 \\ 
 \midrule
 
 \multirowcell{3}{\dataset-S} & all & 12.07 & 36.89 & - & 1.00 & -  \\ 
 & valid & \textbf{12.63} & \textbf{47.78} & 47.78 & 54.77 & 51.04 \\ 
 & invalid & 11.32 & 28.91 & 71.09 & 65.02 & 67.92 \\ 
 \midrule
 
 \multirowcell{3}{\dataset-P} & all & 14.32 & 46.70 & - & 1.00 & -  \\ 
 & valid & \textbf{14.78} & \textbf{52.07} & 52.07 & 63.25 & 57.12 \\ 
 & invalid & 13.56 & 39.66 & 60.34 & 48.98 & 54.07 \\ 
 \midrule
\end{tabular}
\caption{O, BLEU-2 \antoine{need better caption}}
\label{tab:comet-disc-eval}
\end{table}


\begin{table}[t]
% \footnotesize
\small
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|l|lc}

\toprule
\textbf{Event + Rel} & \textbf{Generation} & \textbf{V} & \textbf{C}\\
\midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not skate \\around\\\textbf{\textit{xAttr}}}} & athletic & \xmark & \xmark \\
 & careless & \xmark & \xmark \\
 & lazy & \cmark & \cmark \\
 & uncoordinated & \cmark & \cmark \\
 & unskilled & \cmark & \cmark \\ 
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not sit \\behind Y\\\textbf{\textit{xIntent}}}} & to be alone & \cmark & \cmark \\
 & to be left alone & \cmark & \cmark \\
 & to avoid Y & \cmark & \cmark \\
 & to sit & \xmark & \xmark \\
 & to wait & \cmark & \xmark \\
 \midrule

 \multirow{5}{*}{\makecell[tl]{X does \\not look \\angry\\\textbf{\textit{xNeed}}}} & to calm down & \cmark & \cmark \\
 & to watch a movie & \xmark & \xmark \\
 & to have been provoked & \xmark & \xmark \\
 & to not be angry & \xmark & \cmark \\
 & to be calm & \cmark & \cmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not rent \\an apartment\\\textbf{\textit{xWant}}}} & to save money & \cmark & \cmark \\
 & to get a job & \cmark & \xmark \\
 & to pay rent & \xmark & \xmark \\
 & to move in & \xmark & \xmark \\
 & to get a new apartment & \xmark & \xmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X is \\not offered \\the job\\\textbf{\textit{oWant}}}} & to hire X & \xmark & \xmark \\
 & to fire X & \cmark & \cmark \\
 & to hire someone else & \cmark & \cmark \\
 & to accept the job & \xmark & \xmark \\
 & to hire them & \xmark & \xmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does\\not buy \\a snack\\\textbf{\textit{xReact}}}} & satisfied & \xmark & \xmark\\
 & hungry & \cmark & \cmark\\
 & satiated & \xmark & \xmark\\
 & full & \xmark & \xmark\\
 & guilty & \cmark & \xmark\\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not bring Y\\into conflict\\\textbf{\textit{oWant}}}} & relieved & \cmark & \cmark \\
 & sad & \xmark & \xmark \\
 & satisfied & \cmark & \cmark \\
 & grateful & \cmark & \cmark \\
 & angry & \xmark & \xmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not learn \\new things\\\textbf{\textit{xEffect}}}} & gains knowledge & \xmark & \xmark \\
 & becomes lazy & \cmark & \cmark \\
 & gets bored & \cmark & \cmark \\
 & becomes ignorant & \cmark & \cmark \\
 & cries & \cmark & \cmark \\
 \midrule
 
 \multirow{5}{*}{\makecell[tl]{X does \\not put Y \\in mind\\\textbf{\textit{oEffect}}}} & becomes confused & \xmark & \cmark \\
 & does not think about X & \cmark & \cmark \\
 & Y thinks about X & \xmark & \xmark \\
 & Y is not remembered & \cmark & \cmark \\
 & cries & \xmark & \cmark \\
\bottomrule

\end{tabular}
\caption{Randomly selected generations of the original COMET model regarding logical negation events. The top 5 options are classified as either \textit{valid} or \textit{invalid} by the \textbf{LSP} discriminator. \textbf{V}alid indicates whether a option is classified as \textit{valid} by the \textbf{LSP} discriminator. \textbf{C}orrect indicates whether a option is plausible judging by humans.} 
% }
\label{tab:discriminator-generations-logical}
\end{table}

The BLEU-2 and human evaluation accuracy scores in Table \ref{tab:comet-disc-eval} demonstrate that the overall negation discriminators trained on logical, semi-logical, and pragmatic negation data (\textbf{LSP}) can extract a subset (i.e., the \textit{valid} set) of candidates from the full beam with higher average accuracy for all types of negation and original events while leaving options with lower quality out (i.e., the \textit{invalid} set). 
For the logical and semi-logical negation evaluation sets, recall scores indicate that the discriminator successfully rules out around 65\% of the incorrect candidates from the full beam. Furthermore, about 55\% correct candidates are selected by the \textbf{LSP} discriminator. For the original and pragmatic negation event types for which the logical implication is subtle, about 65\% of correct options and 45\% of incorrect options are successfully identified by the \textbf{LSP} discriminator.
Table \ref{tab:discriminator-generations-logical} shows examples of \textit{valid} and \textit{invalid} candidates for logical negation events as specified by the \textbf{LSP} discriminator.

\begin{table}
% \small
\footnotesize
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{4.5pt}
\centering
\begin{tabular}{l|r|rrrr}
 
 \multicolumn{2}{c|}{\diagbox[width=\widthof{xxxxxxxxxx}]{\textbf{Eval}}{\textbf{Disc}}} & \textbf{L} & \textbf{S} & \textbf{P} & \textbf{LSP} \\ 
 \midrule

 \multirowcell{3}{\atomic} & all & \textbf{55.69} & 55.93 & 56.94 & 58.30 \\ 
 & valid & 55.65 & \textbf{56.18} & \textbf{57.26} & \textbf{59.07} \\ 
 & \%iprv & -0.07 & 0.44 & 0.57 & \underline{1.32} \\ 
 \midrule
 
 \multirowcell{3}{\dataset-L} & all & 39.46 & 37.85 & 36.43 & 39.45 \\ 
 & valid & \textbf{**46.39} & \textbf{**41.93} & \textbf{37.54} & \textbf{**45.59} \\ 
 & \%iprv & \underline{17.55} & 10.78 & 3.03 & 15.57 \\ 
 \midrule
 
 \multirowcell{3}{\dataset-S} & all & 37.13 & 39.29 & 37.72 & 38.55 \\ 
 & valid & \textbf{37.48} & \textbf{**44.58} & \textbf{39.03} & \textbf{**44.93} \\ 
 & \%iprv & 0.96 & 13.47 & 3.45 & \underline{16.56} \\ 
 \midrule
 
 \multirowcell{3}{\dataset-P} & all & \textbf{46.92} & 47.32 & 48.26 & 48.81 \\ 
 & valid & 46.83 & \textbf{47.68} & \textbf{48.79} & \textbf{**51.44} \\ 
 & \%iprv & -0.20 & 0.75 & 1.09 & \underline{5.40} \\ 
 \midrule
\end{tabular}

\caption{For generations of COMET trained on \atomic, the Precision @ \{\# valid\} scores of the \textit{all} and \textit{valid} sets determined by the \textbf{L}, \textbf{S}, \textbf{LP} and \textbf{LSP} discriminators with respect to the original and negation evaluation sets. The double asterisks(**) indicate significant level at 0.01. iprv\% is the percentage improvement of the \textit{valid} set over the \textit{all} set.}
\label{tab:o-p@len(valid)}
\end{table}

To examine the specific contribution of each negation type towards different evaluation sets, we also look at discriminators trained on single type of negation data (i.e., \textbf{L}, \textbf{S}, \textbf{P}) and compare the P@len(valid) score of the \textit{all} and \textit{valid} sets. Table \ref{tab:o-p@len(valid)} shows that the \textbf{L} discriminator achieves significant improvement of P@len(valid) over the logical negation evaluation set at p < 0.01. The \textbf{S} discriminator not only achieves significant improvement over semi-logical negation events but also over logical negation events at p < 0.01, indicating a transfer of learning outcome between negation types. Although the \textbf{P} discriminator does not gain a significant improvement of p@len(valid) over any evaluation set, when combining the pragmatic negation with logical and semi-logical negations in training the \textbf{L+S+P} discriminator, it achieves significant improvement over all three types of negation events at p < 0.01. Results from Table \ref{tab:o-p@len(valid)} indicates that we can apply negation discriminators, particularly the more well-rounded \textbf{LSP} discriminator, as filters to extract a subset of options from raw generations of the original COMET model with better accuracy for negated event queries.

\begin{table}
% \small
\footnotesize
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{4.5pt}
\centering
\begin{tabular}{l|r|rrrr}
 
 \multicolumn{2}{c|}{\diagbox[width=\widthof{xxxxxxxxxx}]{\textbf{Eval}}{\textbf{Disc}}} & \textbf{L} & \textbf{S} & \textbf{P} & \textbf{LSP} \\ 
 \midrule

 \multirowcell{3}{\atomic} & all & 54.16 & 54.49 & 55.03 & 55.68 \\ 
 & valid & \textbf{54.20} & \textbf{54.64} & \textbf{55.71} & \textbf{**57.58} \\ 
 & \%iprv & 0.08 & 0.28 & 1.23 & \underline{3.41} \\ 
 \midrule
 
 \multirowcell{3}{\dataset-L} & all & 46.54 & 46.26 & 46.15 & 46.39 \\ 
 & valid & \textbf{**50.71} & \textbf{**48.36} & \textbf{46.16} & \textbf{**49.85} \\ 
 & \%iprv & \underline{8.98} & 4.54 & 0.03 & 7.45 \\ 
 \midrule
 
 \multirowcell{3}{\dataset-S} & all & 46.90 & 47.73 & 47.47 & 47.53 \\ 
 & valid & \textbf{47.14} & \textbf{**50.42} & \textbf{48.20} & \textbf{**50.62} \\ 
 & \%iprv & 0.51 & 5.65 & 1.55 & \underline{6.50} \\ 
 \midrule
 
 \multirowcell{3}{\dataset-P} & all & 50.80 & 51.29 & 51.28 & 51.83 \\ 
 & valid & \textbf{50.94} & \textbf{51.52} & \textbf{*52.65} & \textbf{**53.91} \\ 
 & \%iprv & 0.28 & 0.45 & 2.67 & \underline{4.02} \\ 
 \midrule
\end{tabular}

\caption{For generations of COMET trained on \textbf{O+L+S+P}, the P@len(valid) scores of the \textit{all} and \textit{valid} sets determined by \textbf{L}, \textbf{S}, \textbf{LP} and \textbf{LSP} discriminators with respect to the original and negation evaluation sets. The single (*) and double asterisks (**) indicate significant level at 0.05 and 0.01 respectively. iprv\% is the percentage improvement of the \textit{valid} set over the \textit{all} set.}
\label{tab:o+l+s+p-p@len(valid)}
\end{table}

Furthermore, we apply negation discriminators to the COMET model trained on negation data and achieve further improvement over the select output set's quality as shown in Table \ref{tab:o+l+s+p-p@len(valid)}. 
By applying the \textbf{LSP} discriminator to generations of COMET model trained on \textbf{O+L+S+P}, it achieves significant improvements over all evaluation sets, including the original events at p < 0.01. 
The \textbf{P} discriminator also achieves significant improvement with respect to pragmatic negation events at P < 0.05, which is not observed when applying it to the generations of COMET trained on \textbf{O}. The full evaluation of the P@len(valid) and P@3 scores of applying different discriminators to generations of COMET trained on different data over all evaluation sets are shown in Table \ref{tab:full-p@len(valid)} and \ref{tab:full-p@3} in Appendix \ref{sec:appendix}.

